Love tHy Neighbour: Remeasuring Local Structural Node Similarity in Hypergraph-Derived Networks

The problem of node-similarity in networks has motivated a plethora of such measures between node-pairs, which make use of the underlying graph structure. However, higher-order relations cannot be losslessly captured by mere graphs and hence, extensions thereof viz. hypergraphs are used instead. Measuring proximity between node pairs in such a setting calls for a revision in the topological measures of similarity, lest the hypergraph structure remains under-exploited. We, in this work, propose a multitude of hypergraph-oriented similarity scores between node-pairs, thereby providing novel solutions to the link prediction problem. As a part of our proposition, we provide theoretical formulations to extend graph-topology based scores to hypergraphs. We compare our scores with graph-based scores (over clique-expansions of hypergraphs into graphs) from the state-of-the-art. Using a combination of the existing graph-based and the proposed hypergraph-based similarity scores as features for a classifier predicts links much better than using the former solely. Experiments on several real-world datasets and both quantitative as well as qualitative analyses on the same exhibit the superiority of the proposed similarity scores over the existing ones.

==> algorithms/data_prep.tex <==
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Temporal Graph $G = (V, E, T)$\newline
       Split ratio $r \in [0, 1]$ \newline
       Sampling factor $p \in \mathbb{R}$}
\Output{Train edges $E_{tr}$\newline
        Test links $E_{te}$ \newline
        Test non-links $\hat{E}_{te}$}
\SetAlgoLined
 $E_{tr}, E_{te} \leftarrow$ \textsc{temporalSplit}($G$, $r$)
 
 $\hat{E}_{te} \leftarrow$ \textsc{sampleNonLinks}($E_{tr}$, $E_{te}$, $p$)
 
 \Return{$E_{tr}$, $E_{te}$, $\hat{E}_{te}$}

==> algorithms/data_prep_hyg.tex <==
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Hypergraph $H$\newline
       Split ratio $r \in [0, 1]$ \newline
       Sampling factor $p \in \mathbb{R}$}
\Output{Train hyperedges $F_{tr}$\newline
        Test links $E_{te}$ \newline
        Test non-links $\hat{E}_{te}$}
% \SetAlgoLined
\DontPrintSemicolon
 \uIf{\textsc{isTemporal}($H$)}{$F_{tr}, E_{te} \leftarrow$ \textsc{temporalSplit}($H$, $r$)}
 \Else{$F_{tr}, E_{te} \leftarrow$ \textsc{structuralSplit}($H$, $r$)}
 $\hat{E}_{te} \leftarrow$ \textsc{sampleNonLinks}($F_{tr}$, $E_{te}$, $p$)
 
 \Return{$F_{tr}$, $E_{te}$, $\hat{E}_{te}$}

==> algorithms/split_train_test.tex <==
\SetCommentSty{mycommfont}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Temporal Graph $G = (V, E, T_E)$\newline
       Split ratio $r \in [0, 1]$}
\Output{Train edges $E_{tr}$\newline
        Test links $E_{te}$}
\DontPrintSemicolon
$\mathcal{R}_{T_E} \leftarrow \{T_E[e] ~|~ e \in E\} \subseteq \mathbb{R}$ %\tcp*{timeline = range of $T_E$}
$\tau_r \leftarrow \mathbf{P}_{r\%}(\mathcal{R}_{T_E})$ %\tcp*{split-threshold = $r\%$ percentile of timeline}
$E_{tr} \leftarrow \{e \in E ~|~ T[e] \leq \tau_r\}$\;
$E_{te} \leftarrow \{e \in E ~|~ T[e] > \tau_r\}$\;
 \Return{$E_{tr}$, $E_{te}$}

==> algorithms/split_train_test_hyg.tex <==
\SetCommentSty{mycommfont}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{ 
    Temporal Hypergraph $H = (V, F, T_F)$\newline
    Split ratio $r \in [0, 1]$
}
\Output{ 
    Train hyperedges $F_{tr}$\newline
    Test links $E_{te}$
}
% \SetAlgoLined
\DontPrintSemicolon
$E \leftarrow \{\}$\; %\tcp*{edges $E$ initialized to be empty-set}
$T_E : E \rightarrow \mathbb{R}$\; %\tcp*{edge-times $T_E$ initialized as empty map}
\For{$f \in F$}{
    \For{$e \in \powerset_2(f)$}{
        \uIf{$e \in E$}{
            $T_E[e] \leftarrow \min\{T_E[e], T_F[f]\}$
        }
        \Else{
            $E \leftarrow E \cup \{e\}$\;
            $T_E[e] \leftarrow T_F[f]$\;
        }
    }
}
$\mathcal{R}_{T_E} \leftarrow \{T_E[e] ~|~ e \in E\} \subseteq \mathbb{R}$\; %\tcp*{timeline = range of $T_E$}
$\tau_r \leftarrow \mathbf{P}_{r\%}(\mathcal{R}_{T_E})$\; %\tcp*{split-threshold = $r\%$ percentile of timeline}
$F_{tr} \leftarrow \{f \in F ~|~ T[f] \leq \tau_r\}$\;
$E_{te} \leftarrow \{e \in E ~|~ T[e] > \tau_r\}$\;
\Return{$F_{tr}$, $E_{te}$}

==> images/data_preparation.tex <==
\smartdiagramset{
module minimum width=2.5cm,
text width=2.5cm,
module x sep=3.25cm,
back arrow disabled=true}
\smartdiagram[flow diagram:horizontal]{{$G = (V, E, T)$\\$G = (V, E)$}, {$r$-split,\\$\sigma_r(E) = (E_{tr}, E_{te})$}, {$p,r$-subsampling, $\psi_{p, r}(E) = \hat{E}_{te}$}, {LP Data:\\$(E_{tr}, E_{te}, \hat{E}_{te})$}}

==> images/data_preparation_hyg.tex <==
\smartdiagramset{
module minimum width=2.5cm,
text width=2.5cm,
module x sep=3.25cm,
back arrow disabled=true}
\smartdiagram[flow diagram:horizontal]{
    {$H = (V, F, T)$\\$H = (V, F)$},
    {$r$-split,\\$\sigma_r(F) = (F_{tr}, E_{te})$},
    {$p,r$-subsampling, $\psi_{p, r}(F) = \hat{E}_{te}$},
    {LP Data:\\$(F_{tr}, E_{te}, \hat{E}_{te})$}}

==> sections/data_prep.tex <==




==> sections/results/link_prediction/structural.tex <==
Tables~\ref{tab:perf:combined:AA/structural_auc}--\ref{tab:perf:combined:Kz/structural_p@+} show link prediction performance measures for graph and hypergraph based scores.
We show the scores separately for each graph-based topological measure.

\begin{table}[H]
    \centering
    \input{tables/perf/combined/AA/structural_auc}
    \caption{Adamic Adar; AUC scores (\%); Structural split}
    \label{tab:perf:combined:AA/structural_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/AA/structural_p@100}
    \caption{Adamic Adar; Precision@100 scores (\%); Structural split}
    \label{tab:perf:combined:AA/structural_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/AA/structural_p@+}
    \caption{Adamic Adar; Precision@+ scores (\%); Structural split}
    \label{tab:perf:combined:AA/structural_p@+}
\end{table}




\begin{table}[H]
    \centering
    \input{tables/perf/combined/AS/structural_auc}
    \caption{Association Strength; AUC scores (\%); Structural split}
    \label{tab:perf:combined:AS/structural_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/AS/structural_p@100}
    \caption{Association Strength; Precision@100 scores (\%); Structural split}
    \label{tab:perf:combined:AS/structural_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/AS/structural_p@+}
    \caption{Association Strength; Precision@+ scores (\%); Structural split}
    \label{tab:perf:combined:AS/structural_p@+}
\end{table}




\begin{table}[H]
    \centering
    \input{tables/perf/combined/CN/structural_auc}
    \caption{Common Neighbor; AUC scores (\%); Structural split}
    \label{tab:perf:combined:CN/structural_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/CN/structural_p@100}
    \caption{Common Neighbor; Precision@100 scores (\%); Structural split}
    \label{tab:perf:combined:CN/structural_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/CN/structural_p@+}
    \caption{Common Neighbor; Precision@+ scores (\%); Structural split}
    \label{tab:perf:combined:CN/structural_p@+}
\end{table}




\begin{table}[H]
    \centering
    \input{tables/perf/combined/JC/structural_auc}
    \caption{Jaccard Coefficient; AUC scores (\%); Structural split}
    \label{tab:perf:combined:JC/structural_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/JC/structural_p@100}
    \caption{Jaccard Coefficient; Precision@100 scores (\%); Structural split}
    \label{tab:perf:combined:JC/structural_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/JC/structural_p@+}
    \caption{Jaccard Coefficient; Precision@+ scores (\%); Structural split}
    \label{tab:perf:combined:JC/structural_p@+}
\end{table}



\begin{table}[H]
    \centering
    \input{tables/perf/combined/Kz/structural_auc}
    \caption{Katz; AUC scores (\%); Structural split}
    \label{tab:perf:combined:Kz/structural_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/Kz/structural_p@100}
    \caption{Katz; Precision@100 scores (\%); Structural split}
    \label{tab:perf:combined:Kz/structural_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/Kz/structural_p@+}
    \caption{Katz; Precision@+ scores (\%); Structural split}
    \label{tab:perf:combined:Kz/structural_p@+}
\end{table}





%%% CLASSIFIER SCORES HERE %%%



\begin{table}[H]
    \centering
    \input{tables/perf/classifier/AA/structural_auc}
    \caption{XGBoost with Adamic Adar; AUC scores (\%); Structural split}
    \label{tab:perf:classifier:AA/structural_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/AA/structural_p@100}
    \caption{XGBoost with Adamic Adar; Precision@100 scores (\%); Structural split}
    \label{tab:perf:classifier:AA/structural_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/AA/structural_p@+}
    \caption{XGBoost with Adamic Adar; Precision@+ scores (\%); Structural split}
    \label{tab:perf:classifier:AA/structural_p@+}
\end{table}




\begin{table}[H]
    \centering
    \input{tables/perf/classifier/AS/structural_auc}
    \caption{XGBoost with Association Strength; AUC scores (\%); Structural split}
    \label{tab:perf:classifier:AS/structural_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/AS/structural_p@100}
    \caption{XGBoost with Association Strength; Precision@100 scores (\%); Structural split}
    \label{tab:perf:classifier:AS/structural_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/AS/structural_p@+}
    \caption{XGBoost with Association Strength; Precision@+ scores (\%); Structural split}
    \label{tab:perf:classifier:AS/structural_p@+}
\end{table}




\begin{table}[H]
    \centering
    \input{tables/perf/classifier/CN/structural_auc}
    \caption{XGBoost with Common Neighbor; AUC scores (\%); Structural split}
    \label{tab:perf:classifier:CN/structural_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/CN/structural_p@100}
    \caption{XGBoost with Common Neighbor; Precision@100 scores (\%); Structural split}
    \label{tab:perf:classifier:CN/structural_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/CN/structural_p@+}
    \caption{XGBoost with Common Neighbor; Precision@+ scores (\%); Structural split}
    \label{tab:perf:classifier:CN/structural_p@+}
\end{table}




\begin{table}[H]
    \centering
    \input{tables/perf/classifier/JC/structural_auc}
    \caption{XGBoost with Jaccard Coefficient; AUC scores (\%); Structural split}
    \label{tab:perf:classifier:JC/structural_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/JC/structural_p@100}
    \caption{XGBoost with Jaccard Coefficient; Precision@100 scores (\%); Structural split}
    \label{tab:perf:classifier:JC/structural_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/JC/structural_p@+}
    \caption{XGBoost with Jaccard Coefficient; Precision@+ scores (\%); Structural split}
    \label{tab:perf:classifier:JC/structural_p@+}
\end{table}



\begin{table}[H]
    \centering
    \input{tables/perf/classifier/Kz/structural_auc}
    \caption{XGBoost with Katz; AUC scores (\%); Structural split}
    \label{tab:perf:classifier:Kz/structural_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/Kz/structural_p@100}
    \caption{XGBoost with Katz; Precision@100 scores (\%); Structural split}
    \label{tab:perf:classifier:Kz/structural_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/Kz/structural_p@+}
    \caption{XGBoost with Katz; Precision@+ scores (\%); Structural split}
    \label{tab:perf:classifier:Kz/structural_p@+}
\end{table}


==> sections/results/link_prediction/temporal.tex <==
Tables~\ref{tab:perf:combined:AA/temporal_auc}--\ref{tab:perf:combined:Kz/temporal_p@100} report the temporal link prediction performance scores for graph- and hypergraph-based topological measures.
Now, combined performance scores for various link prediction scores.

\begin{table}[H]
    \centering
    \input{tables/perf/combined/AA/temporal_auc}
    \caption{Adamic Adar; AUC scores (\%); temporal split}
    \label{tab:perf:combined:AA/temporal_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/AA/temporal_p@100}
    \caption{Adamic Adar; Precision@100 scores (\%); temporal split}
    \label{tab:perf:combined:AA/temporal_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/AA/temporal_p@+}
    \caption{Adamic Adar; Precision@+ scores (\%); temporal split}
    \label{tab:perf:combined:AA/temporal_p@+}
\end{table}




\begin{table}[H]
    \centering
    \input{tables/perf/combined/AS/temporal_auc}
    \caption{Association Strength; AUC scores (\%); temporal split}
    \label{tab:perf:combined:AS/temporal_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/AS/temporal_p@100}
    \caption{Association Strength; Precision@100 scores (\%); temporal split}
    \label{tab:perf:combined:AS/temporal_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/AS/temporal_p@+}
    \caption{Association Strength; Precision@+ scores (\%); temporal split}
    \label{tab:perf:combined:AS/temporal_p@+}
\end{table}




\begin{table}[H]
    \centering
    \input{tables/perf/combined/CN/temporal_auc}
    \caption{Common Neighbor; AUC scores (\%); temporal split}
    \label{tab:perf:combined:CN/temporal_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/CN/temporal_p@100}
    \caption{Common Neighbor; Precision@100 scores (\%); temporal split}
    \label{tab:perf:combined:CN/temporal_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/CN/temporal_p@+}
    \caption{Common Neighbor; Precision@+ scores (\%); temporal split}
    \label{tab:perf:combined:CN/temporal_p@+}
\end{table}




\begin{table}[H]
    \centering
    \input{tables/perf/combined/JC/temporal_auc}
    \caption{Jaccard Coefficient; AUC scores (\%); temporal split}
    \label{tab:perf:combined:JC/temporal_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/JC/temporal_p@100}
    \caption{Jaccard Coefficient; Precision@100 scores (\%); temporal split}
    \label{tab:perf:combined:JC/temporal_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/JC/temporal_p@+}
    \caption{Jaccard Coefficient; Precision@+ scores (\%); temporal split}
    \label{tab:perf:combined:JC/temporal_p@+}
\end{table}



\begin{table}[H]
    \centering
    \input{tables/perf/combined/Kz/temporal_auc}
    \caption{Katz; AUC scores (\%); temporal split}
    \label{tab:perf:combined:Kz/temporal_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/Kz/temporal_p@100}
    \caption{Katz; Precision@100 scores (\%); temporal split}
    \label{tab:perf:combined:Kz/temporal_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/combined/Kz/temporal_p@+}
    \caption{Katz; Precision@+ scores (\%); temporal split}
    \label{tab:perf:combined:Kz/temporal_p@+}
\end{table}


%%% CLASSIFIER SCORES HERE %%%


\begin{table}[H]
    \centering
    \input{tables/perf/classifier/AA/temporal_auc}
    \caption{XGBoost with Adamic Adar; AUC scores (\%); temporal split}
    \label{tab:perf:classifier:AA/temporal_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/AA/temporal_p@100}
    \caption{XGBoost with Adamic Adar; Precision@100 scores (\%); temporal split}
    \label{tab:perf:classifier:AA/temporal_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/AA/temporal_p@+}
    \caption{XGBoost with Adamic Adar; Precision@+ scores (\%); temporal split}
    \label{tab:perf:classifier:AA/temporal_p@+}
\end{table}




\begin{table}[H]
    \centering
    \input{tables/perf/classifier/AS/temporal_auc}
    \caption{XGBoost with Association Strength; AUC scores (\%); temporal split}
    \label{tab:perf:classifier:AS/temporal_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/AS/temporal_p@100}
    \caption{XGBoost with Association Strength; Precision@100 scores (\%); temporal split}
    \label{tab:perf:classifier:AS/temporal_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/AS/temporal_p@+}
    \caption{XGBoost with Association Strength; Precision@+ scores (\%); temporal split}
    \label{tab:perf:classifier:AS/temporal_p@+}
\end{table}




\begin{table}[H]
    \centering
    \input{tables/perf/classifier/CN/temporal_auc}
    \caption{XGBoost with Common Neighbor; AUC scores (\%); temporal split}
    \label{tab:perf:classifier:CN/temporal_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/CN/temporal_p@100}
    \caption{XGBoost with Common Neighbor; Precision@100 scores (\%); temporal split}
    \label{tab:perf:classifier:CN/temporal_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/CN/temporal_p@+}
    \caption{XGBoost with Common Neighbor; Precision@+ scores (\%); temporal split}
    \label{tab:perf:classifier:CN/temporal_p@+}
\end{table}




\begin{table}[H]
    \centering
    \input{tables/perf/classifier/JC/temporal_auc}
    \caption{XGBoost with Jaccard Coefficient; AUC scores (\%); temporal split}
    \label{tab:perf:classifier:JC/temporal_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/JC/temporal_p@100}
    \caption{XGBoost with Jaccard Coefficient; Precision@100 scores (\%); temporal split}
    \label{tab:perf:classifier:JC/temporal_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/JC/temporal_p@+}
    \caption{XGBoost with Jaccard Coefficient; Precision@+ scores (\%); temporal split}
    \label{tab:perf:classifier:JC/temporal_p@+}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/Kz/temporal_auc}
    \caption{XGBoost with Katz; AUC scores (\%); temporal split}
    \label{tab:perf:classifier:Kz/temporal_auc}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/Kz/temporal_p@100}
    \caption{XGBoost with Katz; Precision@100 scores (\%); temporal split}
    \label{tab:perf:classifier:Kz/temporal_p@100}
\end{table}

\begin{table}[H]
    \centering
    \input{tables/perf/classifier/Kz/temporal_p@+}
    \caption{XGBoost with Katz; Precision@+ scores (\%); temporal split}
    \label{tab:perf:classifier:Kz/temporal_p@+}
\end{table}






==> sections/results/node_similarities.tex <==
\subsubsection{Quantitative analysis}

% What we have: For each dataset, a single table of the following variety:
% \begin{table*}[htb]
% \centering
% \caption{Link Prediction Scores for each pair of nodes in a particular dataset.\\
% $|G_i|=10$, $|W_i|=10$, $|H^{(i)}|=40$, $|G_iH^{(i)}|=10$, $|W_iH^{(i)}|=10$, \\
% $|G|=1$, $|W|=1$, $|H|=1$, $|GH|=1$, $|WH| = 1$, $|label| = 1$.\\
% Total 86 columns. One table per 6 datasets.}
% \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
%      \toprule
%      pair & $-G_i-$&
%      $-W_i-$&
%      $-H^{(i)}-$&
%      $-G_iH^{(i)}-$&
%      $-W_iH^{(i)}-$&
%      $-G-$&
%      $-W-$&
%      $-H-$&
%      $-GH-$&
%      $-WH-$&
%       label\\\toprule
%      $u_1, v_1$ &&&&&&&&&&&\\
%      $u_2, v_2$ &&&&&&&&&&&\\
%      $\vdots$   &&&&&&&&&&&\\
%      $u_n, v_n$ &&&&&&&&&&&\\
%      \bottomrule
% \end{tabular}
% \end{table*}


% \begin{table*}[htb]
% \centering
% \caption{AUC performances for ``individual graph topological scores''. Total 8 columns. One table per 6 datasets per 4 performance measures.}
% \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
%      \toprule
%      $i$ & $G_i$&
%      $W_i$&
%      $H_1^{(i)}$&
%      $H_2^{(i)}$&
%      $H_3^{(i)}$&
%      $H_4^{(i)}$&
%      $G_iH^{(i)}$&
%      $W_iH^{(i)}$\\\toprule
%      $AA$ &&&&&&&&&\\
%      $CN$ &&&&&&&&&\\
%      $\vdots$   &&&&&&&&&\\
%      $MaxO$ &&&&&&&&&\\
%      \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table*}[htb]
% \centering
% \caption{AUC performances for ``individual graph topological scores''. Total 9 columns. One table per 6 datasets per 4 performance measures.}
% \begin{tabular}{c|c|c|c|c|c}
%      \toprule
%      dataset & $G$ & $W$ & $H$ & $GH$ & $WH$\\\toprule
%      EmEn &&&&\\
%      CoHiSc &&&&\\
%      NDC-S$\vdots$   &&&&\\
%      NDC-S$MaxO$ &&&&\\
%      \bottomrule
% \end{tabular}
% \end{table*}


\subsubsection{Qualitative analysis}


==> sections/results/temp_tables.tex <==

% \begin{table*}[htb]
%     \caption{standalone rank perf p@+}
%     \label{tab:standalone_rank_perf_p@+}
%     \centering
%     % \footnotesize
%     \input{tables/standalone_rank_perf_p@+.tex}
% \end{table*}

% \begin{table*}[htb]
%     \caption{standalone rank perf r@+}
%     \label{tab:standalone_rank_perf_r@+}
%     \centering
%     % \footnotesize
%     \input{tables/standalone_rank_perf_r@+.tex}
% \end{table*}

% \begin{table*}[htb]
%     \caption{standalone rank perf p@100}
%     \label{tab:standalone_rank_perf_p@100}
%     \centering
%     % \footnotesize
%     \input{tables/standalone_rank_perf_p@100.tex}
% \end{table*}



% \begin{table*}[htb]
%     \caption{standalone perf auc tags-math-sx}
%     \label{tab:standalone_perf_auc_tags-math-sx}
%     \centering
%     % \footnotesize
%     \input{tables/standalone_perf_auc_tags-math-sx.tex}
% \end{table*}

% \begin{table*}[htb]
%     \caption{standalone perf auc threads-math-sx}
%     \label{tab:standalone_perf_auc_threads-math-sx}
%     \centering
%     % \footnotesize
%     \input{tables/standalone_perf_auc_threads-math-sx.tex}
% \end{table*}



% \begin{table*}[htb]
%     \caption{standalone perf auc email-Enron}
%     \label{tab:standalone_perf_auc_email-Enron}
%     \centering
%     % \footnotesize
%     \input{tables/standalone_perf_auc_email-Enron.tex}
% \end{table*}

% \begin{table*}[htb]
%     \caption{standalone perf auc NDC-substances}
%     \label{tab:standalone_perf_auc_NDC-substances}
%     \centering
%     % \footnotesize
%     \input{tables/standalone_perf_auc_NDC-substances}
% \end{table*}

% \begin{table*}[htb]
%     \caption{standalone perf auc coauth-DBLP}
%     \label{tab:standalone_perf_auc_coauth-DBLP}
%     \centering
%     % \footnotesize
%     \input{tables/standalone_perf_auc_coauth-DBLP.tex}
% \end{table*}



% \begin{table*}[htb]
%     \centering
%     \input{tables/perf/email-Enron_temporal/standalone_auc.tex}
%     \caption{email-Enron, temporal, standalone AUC scores}
%     \label{tab:my_label}
% \end{table*}



% \begin{table*}[htb]
%     \caption{micro feat rank perf p@+}
%     \label{tab:micro_feat_rank_perf_p@+}
%     \centering
%     % \footnotesize
%     \input{tables/micro_feat_rank_perf_p@+.tex}
% \end{table*}

% \begin{table*}[htb]
%     \caption{micro feat rank perf r@+}
%     \label{tab:micro_feat_rank_perf_r@+}
%     \centering
%     % \footnotesize
%     \input{tables/micro_feat_rank_perf_r@+.tex}
% \end{table*}

% \begin{table*}[htb]
%     \caption{micro feat rank perf p@100}
%     \label{tab:micro_feat_rank_perf_p@100}
%     \centering
%     % \footnotesize
%     \input{tables/micro_feat_rank_perf_p@100.tex}
% \end{table*}

% \begin{table*}[htb]
%     \caption{micro feat perf auc threads-math-sx}
%     \label{tab:micro_feat_perf_auc_threads-math-sx}
%     \centering
%     % \footnotesize
%     \input{tables/micro_feat_perf_auc_threads-math-sx.tex}
% \end{table*}

% \begin{table*}[htb]
%     \caption{micro feat perf auc tags-math-sx}
%     \label{tab:micro_feat_perf_auc_tags-math-sx}
%     \centering
%     % \footnotesize
%     \input{tables/micro_feat_perf_auc_tags-math-sx.tex}
% \end{table*}

% \begin{table*}[htb]
%     \caption{micro feat perf auc email-Enron}
%     \label{tab:micro_feat_perf_auc_email-Enron}
%     \centering
%     % \footnotesize
%     \input{tables/micro_feat_perf_auc_email-Enron.tex}
% \end{table*}



% \begin{table*}[htb]
%     \caption{micro feat perf auc NDC-substances}
%     \label{tab:micro_feat_perf_auc_NDC-substances}
%     \centering
%     % \footnotesize
%     \input{tables/micro_feat_perf_auc_NDC-substances.tex}
% \end{table*}

% \begin{table*}[htb]
%     \caption{micro feat perf auc coauth-DBLP}
%     \label{tab:micro_feat_perf_auc_coauth-DBLP}
%     \centering
%     % \footnotesize
%     \input{tables/micro_feat_perf_auc_coauth-DBLP.tex}
% \end{table*}




% \begin{table*}[htb]
%     \caption{XGBoost classification p@+ scores for link prediction performed using various feature combinations: \texttt{G}, \texttt{W}, \texttt{H}, \texttt{GH}, \texttt{WH}}
%     \label{tab:macro_feat_perf_auc}
%     \centering
%     % \footnotesize
%     \input{tables/macro_feat_perf_p@+.tex}
% \end{table*}

% \begin{table*}[htb]
%     \caption{XGBoost classification p@100 scores for link prediction performed using various feature combinations: \texttt{G}, \texttt{W}, \texttt{H}, \texttt{GH}, \texttt{WH}}
%     \label{tab:macro_feat_perf_auc}
%     \centering
%     % \footnotesize
%     \input{tables/macro_feat_perf_p@100.tex}
% \end{table*}

% \begin{table*}[htb]
%     \caption{XGBoost classification r@+ scores for link prediction performed using various feature combinations: \texttt{G}, \texttt{W}, \texttt{H}, \texttt{GH}, \texttt{WH}}
%     \label{tab:macro_feat_perf_auc}
%     \centering
%     % \footnotesize
%     \input{tables/macro_feat_perf_r@+.tex}
% \end{table*}

% \begin{table*}[htb]
%     \centering
%     \input{tables/perf/email-Enron_structural/classifier_auc.tex}
%     \caption{email-Enron, structural, classifier AUC scores}
%     \label{tab:my_label}
% \end{table*}

% \begin{table*}[htb]
%     \centering
%     \input{tables/perf/email-Enron_temporal/classifier_auc.tex}
%     \caption{email-Enron, temporal, classifier AUC scores}
%     \label{tab:my_label}
% \end{table*}

% \begin{table*}[htb]
%     \centering
%     \input{tables/perf/email-Enron_temporal/classifier_auc_overfit.tex}
%     \caption{email-Enron, temporal, classifier AUC extent of overfit}
%     \label{tab:my_label}
% \end{table*}





==> tables/matrix_norms.tex <==
\begin{tabular}{ll}
       \toprule
        \textbf{Name} & \textbf{Definition} \\ 
        \toprule
        Max-norm & $\|X\|_{max} := \displaystyle\max_{i, j}\{X_{ij}\}$ \\
        \midrule
        Avg-norm & $\|X\|_{avg} := \displaystyle\frac{1}{m\cdot n}\sum_{i, j} X_{ij}$\\
        \midrule
        L1-norm & $\|X\|_{1} := \displaystyle\sum_{i, j} |X_{ij}|$\\
        \midrule
        L2-norm & $\|X\|_{2} := \sqrt{\displaystyle\sum_{i, j} |X_{ij}|^2}$\\
        \bottomrule
    \end{tabular}

==> tables/micro_feat_perf_auc_NDC-substances.tex <==
\begin{tabular}{lccccc}
\toprule
{} &         \texttt{micro-G} &         \texttt{micro-W} &         \texttt{micro-H} &        \texttt{micro-GH} &        \texttt{micro-WH} \\
\midrule
AA (s)  &           98.5 $\pm$ 0.2 &           98.4 $\pm$ 0.2 &  \textbf{98.6 $\pm$ 0.2} &  \textbf{98.6 $\pm$ 0.2} &  \textbf{98.6 $\pm$ 0.2} \\
AS (s)  &           97.7 $\pm$ 0.2 &           97.7 $\pm$ 0.2 &  \textbf{98.6 $\pm$ 0.2} &  \textbf{98.6 $\pm$ 0.2} &  \textbf{98.6 $\pm$ 0.2} \\
CN (s)  &           98.4 $\pm$ 0.2 &           98.3 $\pm$ 0.2 &           98.5 $\pm$ 0.2 &  \textbf{98.6 $\pm$ 0.2} &  \textbf{98.6 $\pm$ 0.2} \\
Cos (s) &           98.4 $\pm$ 0.2 &           98.3 $\pm$ 0.2 &  \textbf{98.7 $\pm$ 0.2} &  \textbf{98.7 $\pm$ 0.2} &  \textbf{98.7 $\pm$ 0.2} \\
PA (s)  &           97.1 $\pm$ 0.1 &           97.0 $\pm$ 0.1 &           97.2 $\pm$ 0.1 &  \textbf{97.3 $\pm$ 0.1} &  \textbf{97.3 $\pm$ 0.1} \\
JC (s)  &           98.3 $\pm$ 0.2 &           98.1 $\pm$ 0.2 &  \textbf{98.7 $\pm$ 0.2} &  \textbf{98.7 $\pm$ 0.2} &  \textbf{98.7 $\pm$ 0.2} \\
MxO (s) &           98.2 $\pm$ 0.2 &           98.0 $\pm$ 0.2 &           98.6 $\pm$ 0.2 &  \textbf{98.7 $\pm$ 0.2} &  \textbf{98.7 $\pm$ 0.2} \\
MnO (s) &           98.4 $\pm$ 0.2 &           98.2 $\pm$ 0.2 &  \textbf{98.6 $\pm$ 0.2} &  \textbf{98.6 $\pm$ 0.2} &  \textbf{98.6 $\pm$ 0.2} \\
NM (s)  &           98.2 $\pm$ 0.2 &           98.0 $\pm$ 0.2 &  \textbf{98.7 $\pm$ 0.2} &  \textbf{98.7 $\pm$ 0.2} &  \textbf{98.7 $\pm$ 0.2} \\
Prn (s) &           98.4 $\pm$ 0.2 &           98.3 $\pm$ 0.2 &  \textbf{98.7 $\pm$ 0.2} &  \textbf{98.7 $\pm$ 0.2} &  \textbf{98.7 $\pm$ 0.2} \\
AA (t)  &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} \\
AS (t)  &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} \\
CN (t)  &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} \\
Cos (t) &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} \\
PA (t)  &           58.8 $\pm$ 0.1 &           59.1 $\pm$ 0.1 &           61.0 $\pm$ 0.1 &           61.0 $\pm$ 0.1 &  \textbf{61.4 $\pm$ 0.1} \\
JC (t)  &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} \\
MxO (t) &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} \\
MnO (t) &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} \\
NM (t)  &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} \\
Prn (t) &           56.3 $\pm$ 0.1 &           56.2 $\pm$ 0.1 &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} &  \textbf{56.4 $\pm$ 0.1} \\
\bottomrule
\end{tabular}

==> tables/micro_feat_perf_auc_coauth-DBLP.tex <==
\begin{tabular}{lccccc}
\toprule
{} &         \texttt{micro-G} &         \texttt{micro-W} &         \texttt{micro-H} &        \texttt{micro-GH} &        \texttt{micro-WH} \\
\midrule
AA (s)  &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} \\
AS (s)  &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} \\
CN (s)  &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} \\
Cos (s) &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} \\
PA (s)  &           78.9 $\pm$ 0.1 &           78.4 $\pm$ 0.1 &           83.9 $\pm$ 0.1 &  \textbf{84.2 $\pm$ 0.0} &  \textbf{84.2 $\pm$ 0.0} \\
JC (s)  &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} \\
MxO (s) &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} \\
MnO (s) &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} \\
NM (s)  &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} \\
Prn (s) &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} \\
AA (t)  &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} \\
AS (t)  &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} \\
CN (t)  &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} \\
Cos (t) &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} \\
PA (t)  &           82.8 $\pm$ 0.1 &           84.3 $\pm$ 0.1 &           85.8 $\pm$ 0.1 &           85.9 $\pm$ 0.1 &  \textbf{87.2 $\pm$ 0.1} \\
JC (t)  &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} \\
MxO (t) &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} \\
MnO (t) &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} \\
NM (t)  &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} \\
Prn (t) &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} \\
\bottomrule
\end{tabular}

==> tables/micro_feat_perf_auc_tags-math-sx.tex <==
\begin{tabular}{lccccc}
\toprule
{} & \texttt{micro-G} & \texttt{micro-W} &         \texttt{micro-H} &        \texttt{micro-GH} &        \texttt{micro-WH} \\
\midrule
AA (s)  &   94.2 $\pm$ 0.2 &   94.6 $\pm$ 0.2 &  \textbf{95.7 $\pm$ 0.2} &  \textbf{95.7 $\pm$ 0.2} &  \textbf{95.7 $\pm$ 0.2} \\
AS (s)  &   78.7 $\pm$ 0.7 &   76.8 $\pm$ 0.8 &           95.4 $\pm$ 0.2 &  \textbf{95.5 $\pm$ 0.2} &           95.4 $\pm$ 0.2 \\
CN (s)  &   93.4 $\pm$ 0.2 &   94.2 $\pm$ 0.2 &           94.4 $\pm$ 0.2 &  \textbf{94.7 $\pm$ 0.1} &           94.6 $\pm$ 0.2 \\
Cos (s) &   91.7 $\pm$ 0.1 &   90.2 $\pm$ 0.3 &           95.4 $\pm$ 0.2 &  \textbf{95.6 $\pm$ 0.1} &           95.5 $\pm$ 0.2 \\
PA (s)  &   89.5 $\pm$ 0.5 &   88.9 $\pm$ 0.5 &  \textbf{89.8 $\pm$ 0.5} &  \textbf{89.8 $\pm$ 0.5} &  \textbf{89.8 $\pm$ 0.5} \\
JC (s)  &   88.3 $\pm$ 0.1 &   83.8 $\pm$ 0.4 &           95.4 $\pm$ 0.2 &  \textbf{95.5 $\pm$ 0.2} &           95.4 $\pm$ 0.2 \\
MxO (s) &   86.4 $\pm$ 0.2 &   82.8 $\pm$ 0.4 &           95.4 $\pm$ 0.1 &  \textbf{95.5 $\pm$ 0.1} &           95.4 $\pm$ 0.2 \\
MnO (s) &   91.8 $\pm$ 0.1 &   88.7 $\pm$ 0.2 &           94.9 $\pm$ 0.2 &  \textbf{95.1 $\pm$ 0.2} &           94.9 $\pm$ 0.2 \\
NM (s)  &   86.8 $\pm$ 0.1 &   83.0 $\pm$ 0.4 &           95.4 $\pm$ 0.1 &  \textbf{95.5 $\pm$ 0.1} &           95.4 $\pm$ 0.1 \\
Prn (s) &   89.1 $\pm$ 0.3 &   89.6 $\pm$ 0.3 &           95.4 $\pm$ 0.2 &           95.6 $\pm$ 0.1 &  \textbf{95.6 $\pm$ 0.2} \\
AA (t)  &   88.4 $\pm$ 0.6 &   89.5 $\pm$ 0.5 &           89.5 $\pm$ 0.6 &           89.6 $\pm$ 0.7 &  \textbf{90.5 $\pm$ 0.6} \\
AS (t)  &   74.2 $\pm$ 0.6 &   71.7 $\pm$ 0.8 &           89.0 $\pm$ 0.5 &           89.2 $\pm$ 0.5 &  \textbf{89.2 $\pm$ 0.6} \\
CN (t)  &   87.8 $\pm$ 0.6 &   89.4 $\pm$ 0.4 &           88.9 $\pm$ 0.5 &           89.1 $\pm$ 0.5 &  \textbf{90.0 $\pm$ 0.4} \\
Cos (t) &   86.0 $\pm$ 0.7 &   85.0 $\pm$ 0.6 &           89.1 $\pm$ 0.5 &           89.2 $\pm$ 0.5 &  \textbf{89.7 $\pm$ 0.5} \\
PA (t)  &   85.1 $\pm$ 0.6 &   84.7 $\pm$ 0.4 &           85.2 $\pm$ 0.5 &           85.4 $\pm$ 0.5 &  \textbf{85.5 $\pm$ 0.4} \\
JC (t)  &   82.4 $\pm$ 0.8 &   79.3 $\pm$ 0.9 &           89.1 $\pm$ 0.5 &           89.1 $\pm$ 0.5 &  \textbf{89.2 $\pm$ 0.5} \\
MxO (t) &   80.7 $\pm$ 0.8 &   78.3 $\pm$ 0.9 &  \textbf{89.1 $\pm$ 0.6} &           89.1 $\pm$ 0.5 &           89.1 $\pm$ 0.5 \\
MnO (t) &   86.4 $\pm$ 0.7 &   83.8 $\pm$ 0.5 &           89.0 $\pm$ 0.5 &  \textbf{89.4 $\pm$ 0.5} &           89.3 $\pm$ 0.5 \\
NM (t)  &   80.9 $\pm$ 0.9 &   78.5 $\pm$ 0.9 &           89.0 $\pm$ 0.5 &           89.1 $\pm$ 0.5 &  \textbf{89.2 $\pm$ 0.5} \\
Prn (t) &   83.9 $\pm$ 0.6 &   84.4 $\pm$ 0.6 &           89.0 $\pm$ 0.5 &           89.2 $\pm$ 0.5 &  \textbf{89.7 $\pm$ 0.5} \\
\bottomrule
\end{tabular}

==> tables/micro_feat_perf_auc_threads-math-sx.tex <==
\begin{tabular}{lccccc}
\toprule
{} &         \texttt{micro-G} & \texttt{micro-W} &         \texttt{micro-H} &        \texttt{micro-GH} &        \texttt{micro-WH} \\
\midrule
AA (s)  &           89.2 $\pm$ 0.4 &   89.2 $\pm$ 0.4 &  \textbf{89.3 $\pm$ 0.4} &  \textbf{89.3 $\pm$ 0.4} &  \textbf{89.3 $\pm$ 0.4} \\
AS (s)  &           88.9 $\pm$ 0.4 &   88.9 $\pm$ 0.4 &  \textbf{89.3 $\pm$ 0.4} &  \textbf{89.3 $\pm$ 0.4} &  \textbf{89.3 $\pm$ 0.4} \\
CN (s)  &           89.0 $\pm$ 0.4 &   89.0 $\pm$ 0.4 &  \textbf{89.2 $\pm$ 0.4} &  \textbf{89.2 $\pm$ 0.4} &  \textbf{89.2 $\pm$ 0.4} \\
Cos (s) &           88.5 $\pm$ 0.4 &   88.4 $\pm$ 0.4 &  \textbf{89.3 $\pm$ 0.4} &  \textbf{89.3 $\pm$ 0.4} &  \textbf{89.3 $\pm$ 0.4} \\
PA (s)  &           95.4 $\pm$ 0.2 &   95.3 $\pm$ 0.2 &  \textbf{95.5 $\pm$ 0.2} &  \textbf{95.5 $\pm$ 0.2} &  \textbf{95.5 $\pm$ 0.2} \\
JC (s)  &           88.6 $\pm$ 0.4 &   88.5 $\pm$ 0.4 &  \textbf{89.3 $\pm$ 0.4} &  \textbf{89.3 $\pm$ 0.4} &  \textbf{89.3 $\pm$ 0.4} \\
MxO (s) &           88.6 $\pm$ 0.4 &   88.5 $\pm$ 0.4 &  \textbf{89.3 $\pm$ 0.4} &  \textbf{89.3 $\pm$ 0.4} &  \textbf{89.3 $\pm$ 0.4} \\
MnO (s) &           88.8 $\pm$ 0.4 &   88.8 $\pm$ 0.4 &  \textbf{89.3 $\pm$ 0.4} &           89.2 $\pm$ 0.4 &           89.2 $\pm$ 0.4 \\
NM (s)  &           88.3 $\pm$ 0.4 &   88.3 $\pm$ 0.4 &  \textbf{89.3 $\pm$ 0.4} &  \textbf{89.3 $\pm$ 0.4} &  \textbf{89.3 $\pm$ 0.4} \\
Prn (s) &           88.4 $\pm$ 0.4 &   88.4 $\pm$ 0.3 &  \textbf{89.3 $\pm$ 0.4} &  \textbf{89.3 $\pm$ 0.4} &  \textbf{89.3 $\pm$ 0.4} \\
AA (t)  &           69.4 $\pm$ 0.2 &   69.4 $\pm$ 0.2 &           69.8 $\pm$ 0.2 &           69.8 $\pm$ 0.2 &  \textbf{69.9 $\pm$ 0.2} \\
AS (t)  &  \textbf{69.8 $\pm$ 0.2} &   69.7 $\pm$ 0.2 &  \textbf{69.8 $\pm$ 0.2} &  \textbf{69.8 $\pm$ 0.2} &  \textbf{69.8 $\pm$ 0.2} \\
CN (t)  &           69.4 $\pm$ 0.2 &   69.4 $\pm$ 0.2 &           69.8 $\pm$ 0.2 &           69.8 $\pm$ 0.2 &  \textbf{69.9 $\pm$ 0.2} \\
Cos (t) &           69.4 $\pm$ 0.2 &   69.2 $\pm$ 0.2 &           69.8 $\pm$ 0.2 &  \textbf{69.9 $\pm$ 0.2} &  \textbf{69.9 $\pm$ 0.2} \\
PA (t)  &           84.7 $\pm$ 0.3 &   84.9 $\pm$ 0.3 &           90.6 $\pm$ 0.1 &           90.6 $\pm$ 0.1 &  \textbf{90.7 $\pm$ 0.1} \\
JC (t)  &           69.4 $\pm$ 0.2 &   69.3 $\pm$ 0.2 &  \textbf{69.8 $\pm$ 0.2} &  \textbf{69.8 $\pm$ 0.2} &  \textbf{69.8 $\pm$ 0.2} \\
MxO (t) &           69.4 $\pm$ 0.2 &   69.3 $\pm$ 0.2 &  \textbf{69.8 $\pm$ 0.2} &  \textbf{69.8 $\pm$ 0.2} &  \textbf{69.8 $\pm$ 0.2} \\
MnO (t) &           69.3 $\pm$ 0.2 &   69.4 $\pm$ 0.2 &  \textbf{69.9 $\pm$ 0.2} &           69.8 $\pm$ 0.2 &           69.8 $\pm$ 0.2 \\
NM (t)  &           69.3 $\pm$ 0.2 &   69.2 $\pm$ 0.2 &  \textbf{69.8 $\pm$ 0.2} &  \textbf{69.8 $\pm$ 0.2} &  \textbf{69.8 $\pm$ 0.2} \\
Prn (t) &           69.4 $\pm$ 0.2 &   69.2 $\pm$ 0.2 &           69.8 $\pm$ 0.2 &  \textbf{69.9 $\pm$ 0.2} &           69.8 $\pm$ 0.2 \\
\bottomrule
\end{tabular}

==> tables/standalone_perf_auc_NDC-substances.tex <==
\begin{tabular}{lcccccc}
\toprule
{} &         \texttt{stand-G} &         \texttt{stand-W} & \texttt{stand-H\textsubscript{max}} & \texttt{stand-H\textsubscript{avg}} & \texttt{stand-H\textsubscript{L1}} & \texttt{stand-H\textsubscript{L2}} \\
\midrule
AA (s)  &           98.5 $\pm$ 0.1 &           98.5 $\pm$ 0.1 &             \textbf{98.7 $\pm$ 0.1} &                      98.0 $\pm$ 0.1 &                     98.3 $\pm$ 0.1 &                     98.4 $\pm$ 0.1 \\
AS (s)  &           97.5 $\pm$ 0.1 &           97.3 $\pm$ 0.1 &             \textbf{98.6 $\pm$ 0.1} &                      98.0 $\pm$ 0.1 &                     98.3 $\pm$ 0.1 &                     98.4 $\pm$ 0.1 \\
CN (s)  &           98.4 $\pm$ 0.1 &           98.4 $\pm$ 0.1 &             \textbf{98.5 $\pm$ 0.1} &                      97.9 $\pm$ 0.1 &                     98.3 $\pm$ 0.1 &                     98.3 $\pm$ 0.1 \\
Cos (s) &           98.4 $\pm$ 0.1 &           98.4 $\pm$ 0.1 &             \textbf{98.7 $\pm$ 0.1} &                      97.9 $\pm$ 0.1 &                     98.3 $\pm$ 0.1 &                     98.4 $\pm$ 0.1 \\
PA (s)  &  \textbf{97.2 $\pm$ 0.1} &           97.0 $\pm$ 0.1 &                      96.3 $\pm$ 0.1 &                      93.8 $\pm$ 0.1 &                     97.1 $\pm$ 0.1 &                     97.0 $\pm$ 0.1 \\
JC (s)  &           98.3 $\pm$ 0.1 &           98.1 $\pm$ 0.1 &             \textbf{98.7 $\pm$ 0.1} &                      98.0 $\pm$ 0.1 &                     98.3 $\pm$ 0.1 &                     98.4 $\pm$ 0.1 \\
MxO (s) &           98.2 $\pm$ 0.1 &           98.0 $\pm$ 0.1 &             \textbf{98.7 $\pm$ 0.1} &                      98.0 $\pm$ 0.1 &                     98.3 $\pm$ 0.1 &                     98.4 $\pm$ 0.1 \\
MnO (s) &           98.3 $\pm$ 0.0 &           98.2 $\pm$ 0.0 &             \textbf{98.6 $\pm$ 0.1} &                      97.9 $\pm$ 0.1 &                     98.3 $\pm$ 0.1 &                     98.4 $\pm$ 0.1 \\
NM (s)  &           98.2 $\pm$ 0.1 &           98.1 $\pm$ 0.1 &             \textbf{98.7 $\pm$ 0.1} &                      98.0 $\pm$ 0.1 &                     98.3 $\pm$ 0.1 &                     98.4 $\pm$ 0.1 \\
Prn (s) &           98.4 $\pm$ 0.1 &           98.4 $\pm$ 0.1 &             \textbf{98.7 $\pm$ 0.1} &                      97.9 $\pm$ 0.1 &                     98.3 $\pm$ 0.1 &                     98.4 $\pm$ 0.1 \\
AA (t)  &  \textbf{56.3 $\pm$ 0.0} &  \textbf{56.3 $\pm$ 0.0} &                      56.2 $\pm$ 0.0 &                      56.2 $\pm$ 0.0 &                     56.2 $\pm$ 0.0 &                     56.2 $\pm$ 0.0 \\
AS (t)  &           56.2 $\pm$ 0.0 &           56.2 $\pm$ 0.0 &             \textbf{56.3 $\pm$ 0.0} &                      56.2 $\pm$ 0.0 &            \textbf{56.3 $\pm$ 0.0} &            \textbf{56.3 $\pm$ 0.0} \\
CN (t)  &           56.2 $\pm$ 0.0 &  \textbf{56.3 $\pm$ 0.0} &                      56.2 $\pm$ 0.0 &                      56.2 $\pm$ 0.0 &                     56.2 $\pm$ 0.0 &                     56.2 $\pm$ 0.0 \\
Cos (t) &  \textbf{56.3 $\pm$ 0.0} &  \textbf{56.3 $\pm$ 0.0} &             \textbf{56.3 $\pm$ 0.0} &                      56.2 $\pm$ 0.0 &                     56.2 $\pm$ 0.0 &                     56.2 $\pm$ 0.0 \\
PA (t)  &           58.6 $\pm$ 0.0 &           58.7 $\pm$ 0.0 &             \textbf{59.5 $\pm$ 0.0} &             \textbf{59.5 $\pm$ 0.0} &            \textbf{59.5 $\pm$ 0.0} &            \textbf{59.5 $\pm$ 0.0} \\
JC (t)  &  \textbf{56.3 $\pm$ 0.0} &  \textbf{56.3 $\pm$ 0.0} &             \textbf{56.3 $\pm$ 0.0} &                      56.2 $\pm$ 0.0 &                     56.2 $\pm$ 0.0 &                     56.2 $\pm$ 0.0 \\
MxO (t) &  \textbf{56.3 $\pm$ 0.0} &  \textbf{56.3 $\pm$ 0.0} &             \textbf{56.3 $\pm$ 0.0} &                      56.2 $\pm$ 0.0 &                     56.2 $\pm$ 0.0 &            \textbf{56.3 $\pm$ 0.0} \\
MnO (t) &  \textbf{56.2 $\pm$ 0.0} &  \textbf{56.2 $\pm$ 0.0} &             \textbf{56.2 $\pm$ 0.0} &             \textbf{56.2 $\pm$ 0.0} &            \textbf{56.2 $\pm$ 0.0} &            \textbf{56.2 $\pm$ 0.0} \\
NM (t)  &  \textbf{56.3 $\pm$ 0.0} &  \textbf{56.3 $\pm$ 0.0} &             \textbf{56.3 $\pm$ 0.0} &                      56.2 $\pm$ 0.0 &                     56.2 $\pm$ 0.0 &            \textbf{56.3 $\pm$ 0.0} \\
Prn (t) &           56.2 $\pm$ 0.0 &           56.1 $\pm$ 0.0 &             \textbf{56.3 $\pm$ 0.0} &                      56.2 $\pm$ 0.0 &                     56.2 $\pm$ 0.0 &                     56.2 $\pm$ 0.0 \\
\bottomrule
\end{tabular}

==> tables/standalone_perf_auc_coauth-DBLP.tex <==
\begin{tabular}{lcccccc}
\toprule
{} &         \texttt{stand-G} &         \texttt{stand-W} & \texttt{stand-H\textsubscript{max}} & \texttt{stand-H\textsubscript{avg}} & \texttt{stand-H\textsubscript{L1}} & \texttt{stand-H\textsubscript{L2}} \\
\midrule
AA (s)  &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} \\
AS (s)  &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} \\
CN (s)  &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} \\
Cos (s) &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} \\
PA (s)  &           76.6 $\pm$ 0.0 &           76.2 $\pm$ 0.0 &                      69.9 $\pm$ 0.0 &                      56.3 $\pm$ 0.0 &            \textbf{77.2 $\pm$ 0.0} &                     75.7 $\pm$ 0.0 \\
JC (s)  &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} \\
MxO (s) &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} \\
MnO (s) &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} \\
NM (s)  &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} \\
Prn (s) &  \textbf{94.4 $\pm$ 0.0} &  \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &             \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} &            \textbf{94.4 $\pm$ 0.0} \\
AA (t)  &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} \\
AS (t)  &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} \\
CN (t)  &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} \\
Cos (t) &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} \\
PA (t)  &           43.4 $\pm$ 0.0 &  \textbf{44.5 $\pm$ 0.0} &                      38.9 $\pm$ 0.0 &                      33.3 $\pm$ 0.0 &                     42.6 $\pm$ 0.0 &                     41.7 $\pm$ 0.0 \\
JC (t)  &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} \\
MxO (t) &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} \\
MnO (t) &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} \\
NM (t)  &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} \\
Prn (t) &  \textbf{56.8 $\pm$ 0.0} &  \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &             \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} &            \textbf{56.8 $\pm$ 0.0} \\
\bottomrule
\end{tabular}

==> tables/standalone_perf_auc_email-Enron.tex <==
\begin{tabular}{lcccccc}
\toprule
{} &         \texttt{stand-G} &         \texttt{stand-W} & \texttt{stand-H\textsubscript{max}} & \texttt{stand-H\textsubscript{avg}} & \texttt{stand-H\textsubscript{L1}} & \texttt{stand-H\textsubscript{L2}} \\
\midrule
AA (s)  &  \textbf{92.6 $\pm$ 0.9} &           91.7 $\pm$ 1.0 &                      92.6 $\pm$ 0.6 &                      91.7 $\pm$ 1.0 &                     89.4 $\pm$ 0.9 &                     90.2 $\pm$ 0.9 \\
AS (s)  &           90.5 $\pm$ 1.1 &           85.2 $\pm$ 1.2 &                      82.6 $\pm$ 0.7 &             \textbf{92.1 $\pm$ 1.0} &                     90.1 $\pm$ 1.0 &                     91.3 $\pm$ 1.0 \\
CN (s)  &  \textbf{91.8 $\pm$ 0.9} &           91.1 $\pm$ 1.0 &                      90.4 $\pm$ 0.6 &                      91.5 $\pm$ 0.9 &                     89.0 $\pm$ 0.9 &                     89.4 $\pm$ 0.8 \\
Cos (s) &  \textbf{93.6 $\pm$ 0.9} &           93.0 $\pm$ 1.0 &                      92.8 $\pm$ 0.8 &                      91.9 $\pm$ 1.0 &                     89.5 $\pm$ 0.9 &                     90.4 $\pm$ 0.9 \\
PA (s)  &  \textbf{71.6 $\pm$ 0.9} &           68.3 $\pm$ 0.9 &                      65.5 $\pm$ 1.6 &                      61.2 $\pm$ 1.2 &                     69.1 $\pm$ 1.0 &                     68.4 $\pm$ 1.0 \\
JC (s)  &  \textbf{93.4 $\pm$ 0.8} &           92.5 $\pm$ 0.9 &                      92.8 $\pm$ 0.7 &                      92.1 $\pm$ 1.0 &                     89.8 $\pm$ 0.9 &                     90.9 $\pm$ 0.9 \\
MxO (s) &  \textbf{92.8 $\pm$ 0.8} &           91.8 $\pm$ 0.9 &                      92.4 $\pm$ 0.7 &                      92.1 $\pm$ 1.0 &                     89.6 $\pm$ 0.9 &                     90.7 $\pm$ 0.9 \\
MnO (s) &  \textbf{92.6 $\pm$ 1.0} &           89.9 $\pm$ 1.2 &                      91.0 $\pm$ 0.7 &                      91.7 $\pm$ 1.0 &                     89.4 $\pm$ 0.9 &                     90.1 $\pm$ 0.9 \\
NM (s)  &  \textbf{93.2 $\pm$ 0.8} &           92.1 $\pm$ 0.9 &                      92.8 $\pm$ 0.7 &                      92.0 $\pm$ 1.0 &                     89.6 $\pm$ 0.9 &                     90.6 $\pm$ 0.9 \\
Prn (s) &           92.4 $\pm$ 1.2 &           90.3 $\pm$ 1.2 &             \textbf{92.8 $\pm$ 0.8} &                      92.0 $\pm$ 1.0 &                     89.6 $\pm$ 0.9 &                     90.6 $\pm$ 0.9 \\
AA (t)  &           59.8 $\pm$ 0.3 &           63.2 $\pm$ 0.2 &                      61.2 $\pm$ 0.3 &             \textbf{64.8 $\pm$ 0.2} &                     57.6 $\pm$ 0.2 &                     58.7 $\pm$ 0.2 \\
AS (t)  &           64.6 $\pm$ 0.1 &  \textbf{66.5 $\pm$ 0.4} &                      56.3 $\pm$ 0.2 &                      63.1 $\pm$ 0.2 &                     56.7 $\pm$ 0.3 &                     56.7 $\pm$ 0.3 \\
CN (t)  &           59.4 $\pm$ 0.3 &           62.6 $\pm$ 0.2 &                      59.6 $\pm$ 0.3 &             \textbf{64.1 $\pm$ 0.2} &                     57.3 $\pm$ 0.2 &                     58.0 $\pm$ 0.2 \\
Cos (t) &           62.3 $\pm$ 0.2 &  \textbf{67.7 $\pm$ 0.2} &                      57.6 $\pm$ 0.2 &                      64.2 $\pm$ 0.2 &                     56.9 $\pm$ 0.3 &                     57.3 $\pm$ 0.3 \\
PA (t)  &           49.9 $\pm$ 0.3 &           45.8 $\pm$ 0.4 &             \textbf{52.0 $\pm$ 0.3} &                      51.5 $\pm$ 0.3 &                     43.2 $\pm$ 0.4 &                     47.1 $\pm$ 0.4 \\
JC (t)  &           60.6 $\pm$ 0.3 &  \textbf{65.7 $\pm$ 0.2} &                      57.4 $\pm$ 0.2 &                      63.6 $\pm$ 0.2 &                     56.9 $\pm$ 0.3 &                     57.2 $\pm$ 0.3 \\
MxO (t) &           59.5 $\pm$ 0.2 &  \textbf{64.8 $\pm$ 0.2} &                      57.0 $\pm$ 0.2 &                      63.3 $\pm$ 0.2 &                     56.7 $\pm$ 0.3 &                     57.1 $\pm$ 0.3 \\
MnO (t) &           65.4 $\pm$ 0.2 &  \textbf{68.2 $\pm$ 0.3} &                      60.3 $\pm$ 0.2 &                      65.0 $\pm$ 0.2 &                     57.2 $\pm$ 0.3 &                     57.7 $\pm$ 0.3 \\
NM (t)  &           60.0 $\pm$ 0.2 &  \textbf{65.2 $\pm$ 0.2} &                      57.3 $\pm$ 0.2 &                      63.5 $\pm$ 0.2 &                     56.8 $\pm$ 0.3 &                     57.1 $\pm$ 0.3 \\
Prn (t) &           64.4 $\pm$ 0.1 &  \textbf{68.9 $\pm$ 0.1} &                      56.8 $\pm$ 0.2 &                      63.0 $\pm$ 0.1 &                     56.5 $\pm$ 0.3 &                     56.7 $\pm$ 0.3 \\
\bottomrule
\end{tabular}

==> tables/standalone_perf_auc_tags-math-sx.tex <==
\begin{tabular}{lcccccc}
\toprule
{} &         \texttt{stand-G} &         \texttt{stand-W} & \texttt{stand-H\textsubscript{max}} & \texttt{stand-H\textsubscript{avg}} & \texttt{stand-H\textsubscript{L1}} & \texttt{stand-H\textsubscript{L2}} \\
\midrule
AA (s)  &           94.3 $\pm$ 0.1 &           94.8 $\pm$ 0.1 &                      94.7 $\pm$ 0.1 &                      83.7 $\pm$ 0.2 &                     94.6 $\pm$ 0.2 &            \textbf{95.0 $\pm$ 0.2} \\
AS (s)  &           67.4 $\pm$ 0.2 &           65.6 $\pm$ 0.2 &                      88.0 $\pm$ 0.2 &                      82.6 $\pm$ 0.3 &                     94.5 $\pm$ 0.2 &            \textbf{94.8 $\pm$ 0.1} \\
CN (s)  &           93.7 $\pm$ 0.2 &  \textbf{94.4 $\pm$ 0.2} &                      90.4 $\pm$ 0.2 &                      83.2 $\pm$ 0.2 &                     94.3 $\pm$ 0.2 &                     94.3 $\pm$ 0.2 \\
Cos (s) &           91.9 $\pm$ 0.1 &           90.3 $\pm$ 0.1 &                      93.9 $\pm$ 0.1 &                      82.9 $\pm$ 0.3 &                     94.4 $\pm$ 0.2 &            \textbf{94.6 $\pm$ 0.2} \\
PA (s)  &  \textbf{89.7 $\pm$ 0.2} &           89.0 $\pm$ 0.2 &                      77.2 $\pm$ 0.5 &                      63.5 $\pm$ 0.4 &                     89.6 $\pm$ 0.2 &                     89.4 $\pm$ 0.2 \\
JC (s)  &           88.5 $\pm$ 0.0 &           84.2 $\pm$ 0.1 &                      93.9 $\pm$ 0.1 &                      83.0 $\pm$ 0.3 &                     94.5 $\pm$ 0.2 &            \textbf{94.7 $\pm$ 0.2} \\
MxO (s) &           86.1 $\pm$ 0.0 &           83.1 $\pm$ 0.1 &                      93.5 $\pm$ 0.1 &                      83.1 $\pm$ 0.3 &                     94.4 $\pm$ 0.2 &            \textbf{94.6 $\pm$ 0.2} \\
MnO (s) &           89.3 $\pm$ 0.2 &           87.6 $\pm$ 0.1 &                      91.3 $\pm$ 0.2 &                      82.8 $\pm$ 0.3 &                     94.4 $\pm$ 0.2 &            \textbf{94.6 $\pm$ 0.1} \\
NM (s)  &           87.2 $\pm$ 0.0 &           83.4 $\pm$ 0.1 &                      93.9 $\pm$ 0.1 &                      83.0 $\pm$ 0.3 &                     94.4 $\pm$ 0.2 &            \textbf{94.6 $\pm$ 0.2} \\
Prn (s) &           89.3 $\pm$ 0.1 &           89.7 $\pm$ 0.2 &                      94.0 $\pm$ 0.1 &                      82.9 $\pm$ 0.3 &                     94.4 $\pm$ 0.2 &            \textbf{94.6 $\pm$ 0.2} \\
AA (t)  &           88.5 $\pm$ 0.1 &  \textbf{89.9 $\pm$ 0.1} &                      87.9 $\pm$ 0.1 &                      79.0 $\pm$ 0.2 &                     89.2 $\pm$ 0.1 &                     89.4 $\pm$ 0.1 \\
AS (t)  &           66.2 $\pm$ 0.1 &           65.0 $\pm$ 0.2 &                      84.1 $\pm$ 0.2 &                      78.3 $\pm$ 0.2 &            \textbf{89.1 $\pm$ 0.1} &            \textbf{89.1 $\pm$ 0.1} \\
CN (t)  &           88.1 $\pm$ 0.1 &  \textbf{89.6 $\pm$ 0.1} &                      84.8 $\pm$ 0.1 &                      78.9 $\pm$ 0.1 &                     89.0 $\pm$ 0.1 &                     89.0 $\pm$ 0.1 \\
Cos (t) &           86.2 $\pm$ 0.1 &           85.4 $\pm$ 0.1 &                      86.9 $\pm$ 0.1 &                      78.6 $\pm$ 0.2 &            \textbf{89.1 $\pm$ 0.1} &            \textbf{89.1 $\pm$ 0.1} \\
PA (t)  &  \textbf{84.0 $\pm$ 0.1} &           83.7 $\pm$ 0.1 &                      63.3 $\pm$ 0.0 &                      61.3 $\pm$ 0.1 &            \textbf{84.0 $\pm$ 0.1} &                     83.7 $\pm$ 0.1 \\
JC (t)  &           82.5 $\pm$ 0.1 &           79.9 $\pm$ 0.1 &                      86.9 $\pm$ 0.1 &                      78.6 $\pm$ 0.2 &            \textbf{89.1 $\pm$ 0.1} &            \textbf{89.1 $\pm$ 0.1} \\
MxO (t) &           80.3 $\pm$ 0.1 &           78.9 $\pm$ 0.1 &                      86.6 $\pm$ 0.1 &                      78.7 $\pm$ 0.1 &                     89.0 $\pm$ 0.1 &            \textbf{89.1 $\pm$ 0.1} \\
MnO (t) &           84.5 $\pm$ 0.1 &           83.3 $\pm$ 0.1 &                      85.4 $\pm$ 0.1 &                      78.4 $\pm$ 0.2 &            \textbf{89.1 $\pm$ 0.1} &            \textbf{89.1 $\pm$ 0.1} \\
NM (t)  &           81.3 $\pm$ 0.1 &           79.2 $\pm$ 0.1 &                      87.0 $\pm$ 0.1 &                      78.6 $\pm$ 0.2 &            \textbf{89.1 $\pm$ 0.1} &            \textbf{89.1 $\pm$ 0.1} \\
Prn (t) &           84.1 $\pm$ 0.1 &           84.9 $\pm$ 0.1 &                      86.9 $\pm$ 0.1 &                      78.6 $\pm$ 0.2 &            \textbf{89.1 $\pm$ 0.1} &            \textbf{89.1 $\pm$ 0.1} \\
\bottomrule
\end{tabular}

==> tables/standalone_perf_auc_threads-math-sx.tex <==
\begin{tabular}{lcccccc}
\toprule
{} &         \texttt{stand-G} &         \texttt{stand-W} & \texttt{stand-H\textsubscript{max}} & \texttt{stand-H\textsubscript{avg}} & \texttt{stand-H\textsubscript{L1}} & \texttt{stand-H\textsubscript{L2}} \\
\midrule
AA (s)  &  \textbf{89.3 $\pm$ 0.1} &  \textbf{89.3 $\pm$ 0.1} &             \textbf{89.3 $\pm$ 0.1} &                      87.5 $\pm$ 0.1 &                     89.2 $\pm$ 0.1 &            \textbf{89.3 $\pm$ 0.1} \\
AS (s)  &           87.3 $\pm$ 0.1 &           87.3 $\pm$ 0.1 &                      89.0 $\pm$ 0.1 &                      87.5 $\pm$ 0.1 &            \textbf{89.2 $\pm$ 0.1} &            \textbf{89.2 $\pm$ 0.1} \\
CN (s)  &  \textbf{89.1 $\pm$ 0.1} &  \textbf{89.1 $\pm$ 0.1} &                      88.6 $\pm$ 0.1 &                      87.5 $\pm$ 0.1 &            \textbf{89.1 $\pm$ 0.1} &            \textbf{89.1 $\pm$ 0.1} \\
Cos (s) &           87.9 $\pm$ 0.1 &           88.1 $\pm$ 0.1 &             \textbf{89.2 $\pm$ 0.1} &                      87.5 $\pm$ 0.1 &            \textbf{89.2 $\pm$ 0.1} &            \textbf{89.2 $\pm$ 0.1} \\
PA (s)  &  \textbf{90.2 $\pm$ 0.1} &           90.1 $\pm$ 0.1 &                      86.8 $\pm$ 0.1 &                      71.9 $\pm$ 0.3 &            \textbf{90.2 $\pm$ 0.1} &                     90.0 $\pm$ 0.1 \\
JC (s)  &           87.9 $\pm$ 0.1 &           88.0 $\pm$ 0.1 &             \textbf{89.2 $\pm$ 0.1} &                      87.5 $\pm$ 0.1 &            \textbf{89.2 $\pm$ 0.1} &            \textbf{89.2 $\pm$ 0.1} \\
MxO (s) &           87.9 $\pm$ 0.1 &           87.9 $\pm$ 0.1 &                      89.1 $\pm$ 0.1 &                      87.5 $\pm$ 0.1 &            \textbf{89.2 $\pm$ 0.1} &            \textbf{89.2 $\pm$ 0.1} \\
MnO (s) &           88.1 $\pm$ 0.1 &           88.4 $\pm$ 0.1 &                      88.8 $\pm$ 0.1 &                      87.5 $\pm$ 0.1 &            \textbf{89.1 $\pm$ 0.1} &            \textbf{89.1 $\pm$ 0.1} \\
NM (s)  &           87.9 $\pm$ 0.1 &           87.9 $\pm$ 0.1 &             \textbf{89.2 $\pm$ 0.1} &                      87.5 $\pm$ 0.1 &            \textbf{89.2 $\pm$ 0.1} &            \textbf{89.2 $\pm$ 0.1} \\
Prn (s) &           87.9 $\pm$ 0.1 &           88.1 $\pm$ 0.1 &             \textbf{89.2 $\pm$ 0.1} &                      87.5 $\pm$ 0.1 &            \textbf{89.2 $\pm$ 0.1} &            \textbf{89.2 $\pm$ 0.1} \\
AA (t)  &  \textbf{69.3 $\pm$ 0.0} &  \textbf{69.3 $\pm$ 0.0} &                      69.2 $\pm$ 0.0 &                      68.6 $\pm$ 0.0 &            \textbf{69.3 $\pm$ 0.0} &            \textbf{69.3 $\pm$ 0.0} \\
AS (t)  &           68.5 $\pm$ 0.0 &           68.5 $\pm$ 0.0 &                      69.0 $\pm$ 0.0 &                      68.6 $\pm$ 0.0 &            \textbf{69.2 $\pm$ 0.0} &            \textbf{69.2 $\pm$ 0.0} \\
CN (t)  &  \textbf{69.3 $\pm$ 0.0} &  \textbf{69.3 $\pm$ 0.0} &                      69.0 $\pm$ 0.0 &                      68.6 $\pm$ 0.0 &            \textbf{69.3 $\pm$ 0.0} &            \textbf{69.3 $\pm$ 0.0} \\
Cos (t) &           68.7 $\pm$ 0.0 &           68.9 $\pm$ 0.0 &                      69.0 $\pm$ 0.0 &                      68.6 $\pm$ 0.0 &            \textbf{69.3 $\pm$ 0.0} &                     69.2 $\pm$ 0.0 \\
PA (t)  &  \textbf{65.7 $\pm$ 0.0} &  \textbf{65.7 $\pm$ 0.0} &                      60.2 $\pm$ 0.0 &                      54.6 $\pm$ 0.0 &                     61.6 $\pm$ 0.0 &                     61.5 $\pm$ 0.0 \\
JC (t)  &           68.7 $\pm$ 0.0 &           68.8 $\pm$ 0.0 &                      69.0 $\pm$ 0.0 &                      68.6 $\pm$ 0.0 &            \textbf{69.3 $\pm$ 0.0} &                     69.2 $\pm$ 0.0 \\
MxO (t) &           68.8 $\pm$ 0.0 &           68.8 $\pm$ 0.0 &                      69.1 $\pm$ 0.0 &                      68.6 $\pm$ 0.0 &            \textbf{69.3 $\pm$ 0.0} &                     69.2 $\pm$ 0.0 \\
MnO (t) &           68.8 $\pm$ 0.0 &           69.0 $\pm$ 0.0 &                      69.0 $\pm$ 0.0 &                      68.6 $\pm$ 0.0 &            \textbf{69.3 $\pm$ 0.0} &                     69.2 $\pm$ 0.0 \\
NM (t)  &           68.8 $\pm$ 0.0 &           68.8 $\pm$ 0.0 &                      69.1 $\pm$ 0.0 &                      68.6 $\pm$ 0.0 &            \textbf{69.3 $\pm$ 0.0} &                     69.2 $\pm$ 0.0 \\
Prn (t) &           68.7 $\pm$ 0.0 &           68.9 $\pm$ 0.0 &                      69.0 $\pm$ 0.0 &                      68.6 $\pm$ 0.0 &            \textbf{69.3 $\pm$ 0.0} &                     69.2 $\pm$ 0.0 \\
\bottomrule
\end{tabular}
